Deep Quantum Circuit Simulations of Low-Energy Nuclear States

Numerical simulation is an important method for verifying the quantum circuits used to simulate low-energy nuclear states. However, real-world applications of quantum computing for nuclear theory often generate deep quantum circuits that place demanding memory and processing requirements on conventional simulation methods. Here, we present advances in high-performance numerical simulations of deep quantum circuits to efficiently verify the accuracy of low-energy nuclear physics applications. Our approach employs several novel methods for accelerating the numerical simulation including 1- and 2-qubit gate fusion techniques as well as management of simulated mid-circuit measurements to verify state preparation circuits. We test these methods across a variety of high-performance computing systems and our results show that circuits up to 21 qubits and more than 115,000,000 gates can be efficiently simulated.

==> tex/6_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

Zhang et al.~have presented a review of selected topics in quantum simulation for nuclear physics \cite{Zhang_2021}. de Jong et al. studied non-equilibrium dynamics derived from the Schwinger model on quantum computer \cite{PhysRevD.106.054508}.


UniQ~\cite{zhang2022uniq} proposes QTensor, a unified intermediate representation for different quantum circuit simulations. For Density matrix simulation, different shapes of Tensors are used in the Kraus and gate operations. It also provides a unified hierarchical hardware abstraction to map the simulation workload to various devices. In particular, it leverages the optimization techniques performed in HyQuas~\cite{zhang2021hyquas}, namely TransMM method, OShareMem method, and global-local swap method, to automatically partition a given circuit into different groups and decide the allocation of the workloads on backend GPUs for better performance.

\textcolor{red}{Works to be inlcuded here: PRX TPU simulation work, SV-Sim/DM-Sim, TVQVM}

==> tex/backup.tex <==
\begin{figure*}[!h]
     \centering
     \begin{subfigure}[h]{0.49\textwidth}
         \centering
    \includegraphics[width=\textwidth]{figure/gate_fusion.pdf}
         \caption{Gate count reduction.}
         \label{fig:gate_count_red}
     \end{subfigure}
     \hfill
     \begin{subfigure}[h]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/gate_fusion_sim.pdf}
         \caption{Simulation time reduction.}
         \label{fig:res_gate_fusion}
     \end{subfigure}
        \caption{The reduction of gate count and the  improvement simulation performance through the 4 gate fusion steps in Section~\ref{subsec:gate_fusion} and Fig.~\ref{fig:gate_fusion_path}.}
    \label{fig:res_gate_fusion_sim}
\end{figure*}



\begin{figure*}[!h]
     \centering
     \begin{subfigure}[h]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/across_plat.pdf}
         \caption{Simulation time for P3 across CPUs and GPUs of Perlmutter, Summit and Crusher.}
         \label{fig:cross_plat}
     \end{subfigure}
     \hfill
     \begin{subfigure}[h]{0.37\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figure/gpu_n20.pdf}
         \caption{Simulation time for P4 and P5 on the three GPUs.}
         \label{fig:gpu_n20}
     \end{subfigure}
        \caption{\textcolor{red}{Fix here. There is no figure caption.}}
        %\label{fig:res_gate_fusion_sim}
\end{figure*}





\vspace{4pt}\noindent\textbf{(ii) Mid-Circuit Measurement Assertion:} We use P5 as the exemplar problem for this evaluation. Shown in  Listing~\ref{lst:qasm}, the projection circuit includes a series of mid-circuit ancilla measurements to amplify the probability of the ground state, given the measurement result is 0. However, it is also possible that the measurement gives 1, which implies that the present shot fails to project to the correct state, seen as a rejection. As shown in Table~\ref{tab:prsetting}, the filtering steps for P5 is 8, implying 8 mid-circuit measurements, labeled as M1 to M8. In Table~\ref{tab:mma}, we repeat three simulations (Case-1 to 3) of the P5 circuit on a Perlmutter A100 GPU using 1024 shots without applying mid-circuit measurement assertion. The values under M1 to M8 show the number of rejected shots during each mid-circuit measurement. 

\begin{table}[!t]
\centering\footnotesize
\caption{Evaluation results for mid-circuit measurement assertion on P5.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline\hline
 & M1 & M2 & M3 & M4 & M5 & M6 & M7 & M8 & Success & Time(ms)  \\ \hline
Case-1 & 403 & 94 & 111 & 43 & 31 & 16 & 28 & 0 & 298  & 379404 \\ \hline
Case-2 & 396 & 89 & 119 & 48 & 36 & 15 & 24 & 0 & 297 & 381236 \\ \hline
Case-3 & 392 & 111 & 126 & 48 & 45 & 11 & 28 & 0 & 263 & 363883  \\ \hline


MMA & 0.60271 & 0.84572 & 0.76447 & 0.88251 & 0.90075 & 0.95215 & 0.92406 & 0.99998 & 0.27253 & 672.777 \\ 
\hline\hline
\end{tabular}
\label{tab:mma}
\end{table}

Within the three trails, for P5, on average 286 of the 1024 shots can project to the final state of interest, implying a  sampling efficiency of 28\% for the projection algorithm. However, because of repeated end-to-end runs due to mid-circuit measurement, the simulation time even on an A100 GPU is still quite significant, on-average 375s. By applying mid-circuit measurement assertion, despite the probability of measuring all-zero is still relatively low, we can always assert it measures 0 and tracking the probability. 

The last row of Table~\ref{tab:mma} shows the ground truth probability of measuring 0 during each mid-circuit measurement. Overall, the probability of obtaining all 0s for M1 to M8 is $27.3\%$. With mid-circuit measurement assertion, we can assert the probability, and ensure the ground state being well-prepared. We can then sample the state by 1024 shots at once in parallel, providing 1024 effective samples. Comparatively, to obtain the same number of effective samples, the original method would need $1024/0.27253=3757$ shots on average and have to be executed sequentially due to mid-circuit measurement.

Overall, the simulation time with MMA is  673ms, 557$\times$ faster than the baseline. When demanding the same number of effective samples, e.g., 1024, the speedup is nearly 2000$\times$. Although the benefit is circuit dependent, it confirms the usefulness and effectiveness of mid-circuit measurement assertion. For problem instances with even lower success rate, e.g., P9 to P15 in Table~\ref{tab:energy}, the gains can be even more extraordinary.

